Self-injective artin algebras without short cycles in the component quiver

We give a complete description of all self-injective artin algebras of infinite representation type whose component quiver has no short cycles.

==> graphs-tikz.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \LinGraph{'iloœæ wierzcho³ków'}{'waulacje'} ' rysuje graf liniowy
\newcommand{\LinGraph}[2]
{
\begin{center}
\begin{tikzpicture}
\foreach \x in {1,...,#1} { \node (e\x) at (2*\x,0) {$\bullet$}; }%

\foreach \x in {2,...,#1} {%
\pgfmathparse{int(\x-1)}\let\y\pgfmathresult;%
\draw[-] (e\x)--(e\y) node[pos=.5,sloped,above] {\foreach
\i/\j/\valA/\valB in #2
{\ifthenelse{\IfVal{\j}{\x}{\i}{\y}}{$(\valA,\valB)$}{}}}; }
\end{tikzpicture}
\end{center}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \DGraph{'iloœæ wierzcho³ków'}{'waulacje'} ' rysuje graf postaci D_n, ale z waluacjami
\newcommand{\DGraph}[2]
{
\begin{center}
\begin{tikzpicture}[scale=0.8]
\pgfmathparse{int(#1)}\let\c\pgfmathresult;%
\pgfmathparse{int(#1-1)}\let\b\pgfmathresult;%
\pgfmathparse{int(#1-2)}\let\a\pgfmathresult;%
\foreach \x in {1,...,\a} { \node (e\x) at (2*\x,0) {$\bullet$}; }%
\node (e\b) at (2*\b,1.5) {$\bullet$};
\node (e\c) at (2*\b,-1.5) {$\bullet$};

\foreach \x in {2,...,\a} {%
\pgfmathparse{int(\x-1)}\let\y\pgfmathresult;%
\draw[-] (e\x)--(e\y) node[pos=.5,sloped,above] {\foreach
\i/\j/\valA/\valB in #2
{\ifthenelse{\IfVal{\j}{\x}{\i}{\y}}{$(\valA,\valB)$}{}}}; }
\draw[-] (e\c)--(e\a);
\draw[-] (e\b)--(e\a);
\end{tikzpicture}
\end{center}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \Can12{'iloœæ wierzcho³ków'} ' rysuje ko³czan algebry kanonicznej, korangi 1 (A), z waluacjami 2,1 oraz 1,2 (parametr 0) lub 1,2 oraz 2,1 (parametr 1)

\newcommand{\CanA}[2]
{
\begin{tikzpicture}[scale=.666]
\pgfmathparse{int(#1)}\let\x\pgfmathresult;%
\pgfmathparse{int(#1-1)}\let\y\pgfmathresult;%
\pgfmathparse{int(#1-2)}\let\z\pgfmathresult;%

% Ustaw 2 wierzcho³ki skrajne oraz jeden na dolnej ga³êzi
\node (c1) at (\x,0) {$\bullet$};
\node (c\y) at (0,0) {$\bullet$};
\node (c\x) at (\x/2,-1.5) {$\bullet$};

% Ustaw #1-2 wierzcho³ków na górnej ga³êzi, co \x/(iloœæ wierzcho³ków w górnej drodze + 1)
\foreach \i in {2,...,\z} { \pgfmathparse{int(\i-1)}\let\a\pgfmathresult; \node (c\i) at (\x-\a*\x/\z,1.5) {$\bullet$}; }%

%Rysujemy strza³ki górnej ga³êzi
\foreach \i in {1,...,\z} {\pgfmathparse{int(\i+1)}\let\a\pgfmathresult; \draw[-latex] (c\i)--(c\a);}
%Rysujemy strza³ki dolnej ga³êzi
\draw[-latex] (c1)--(c\x) node[pos=.5,sloped,above] {\ifthenelse{#2=0}{$(1,2)$}{$(2,1)$}};
\draw[-latex] (c\x)--(c\y) node[pos=.5,sloped,above] {\ifthenelse{#2=0}{$(2,1)$}{$(1,2)$}};

\end{tikzpicture}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \F{'iloœæ wierzcho³ków'} ' rysuje ko³czan algebry kanonicznej, korangi 1 (A), z waluacjami 2,1 oraz 1,2 (parametr 0) lub 1,2 oraz 2,1 (parametr 1)
